PARE: Part Attention Regressor for 3D Human Body Estimation

Despite significant progress, we show that state of the art 3D human pose and shape estimation methods remain sensitive to partial occlusion and can produce dramatically wrong predictions although much of the body is observable. To address this, we introduce a soft attention mechanism, called the Part Attention REgressor (PARE), that learns to predict body-part-guided attention masks. We observe that state-of-the-art methods rely on global feature representations, making them sensitive to even small occlusions. In contrast, PARE's part-guided attention mechanism overcomes these issues by exploiting information about the visibility of individual body parts while leveraging information from neighboring body-parts to predict occluded parts. We show qualitatively that PARE learns sensible attention masks, and quantitative evaluation confirms that PARE achieves more accurate and robust reconstruction results than existing approaches on both occlusion-specific and standard benchmarks. The code and data are available for research purposes at {\small \url{https://pare.is.tue.mpg.de/}}

==> tables/supmat_table_1.tex <==
\paragraph{Comparing to state-of-the-art Temporal Models.}
\begin{table}[h]
	\centering
	\resizebox{0.42\textwidth}{!}{
		\begin{tabular}{ll|r|r}
			\toprule
			& & \multicolumn{2}{c}{ \threedpw }  \\
			\cmidrule(lr){3-4}
			& \bf Method & MPJPE $\downarrow$ & PA-MPJPE $\downarrow$ \\
			\midrule
			\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Temporal}}} & HMMR~\cite{kanazawa_hmr} & 116.5 & 72.6  \\
			& Doersch~\etal~\cite{doersch_sim2real} & - & 74.7 \\
			& Sun~\etal~\cite{Sun_2019_ICCV} & - & 69.5 \\
			& VIBE~\cite{kocabas2019vibe} & 93.5 & 56.5  \\
			& MEVA~\cite{Luo2020MEVA} & 86.9 & 54.7 \\
			\midrule
			& PARE (ResNet-50) & 84.3 & 51.2  \\
			& PARE (HRNet-W32) & \bf 84.1 & \bf 49.3  \\
			\bottomrule
		\end{tabular} 
	}
	\caption{\textbf{Evaluation on the \threedpw dataset.} The numbers are average joint errors in mm. PARE models outperform video-based methods which leverage temporal information.}
    \label{tab:sota_video}
    \vspace{-2ex}
\end{table}{}

==> tables/table_1_3dpw_sota.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.45\textwidth}{!}{
		\begin{tabular}{ll|r|r|r}
			\toprule
			& & \multicolumn{3}{c}{ \threedpw }  \\
			\cmidrule(lr){3-5}
			& \bf Method & MPJPE $\downarrow$ & PA-MPJPE $\downarrow$ & PVE $\downarrow$\\
			\midrule
			\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{temporal}}} & HMMR~\cite{kanazawa_hmr} & 116.5 & 72.6 & - \\
			& Doersch~\etal~\cite{doersch_sim2real} & - & 74.7 & - \\
			& Sun~\etal~\cite{Sun_2019_ICCV} & - & 69.5 & - \\
			& VIBE~\cite{kocabas2019vibe} & 93.5 & 56.5 & 113.4 \\
			& MEVA~\cite{Luo2020MEVA} & 86.9 & 54.7 & - \\
			\midrule
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{multi stage}}} & Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & 89.2 & 58.9 & - \\
			& Zanfir~\etal~\cite{zanfir2020weakly} & 90.0 & 57.1 & - \\
			& I2L-MeshNet~\cite{Moon_2020_ECCV_I2L-MeshNet} & 93.2 & 58.6  & - \\
			& LearnedGD~\cite{song2020human} & - & 56.4  & - \\
			\midrule
			\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{single stage}}} & HMR~\cite{kanazawa_hmr} & 130.0 & 76.7  & \\
			& CMR~\cite{kolotouros2019cmr} & - & 70.2  & - \\
			& SPIN~\cite{SPIN:ICCV:2019} & 96.9 & 59.2  & 135.1 \\
			& HMR-EFT~\cite{joo2020eft} & - & 54.2  & - \\
% 			& HybrIK~\cite{li2021hybrik} & 80.1 & 48.8 & 94.5 \\
% 			& METRO~\cite{lin2021metro} & \textbf{77.1} & 47.9 & \textbf{88.2} \\
			\cmidrule(lr){2-5}
			& PARE (R50) & 84.3 & 51.2  & 101.2 \\
			% & PARE (R50) w. 3DPW & - & -  & - \\
			& PARE (HRNet-W32) & 84.1 & 49.3  & 99.4 \\
			& PARE (HRNet-W32) w. 3DPW & \textbf{79.1} & \textbf{46.4} & \textbf{94.2} \\
			\bottomrule
		\end{tabular} 
	}
	\vspace{-0.05in}
	\caption{\textbf{Evaluation on the \threedpw dataset.} The numbers are average joint errors and average vertex error in mm. PARE models outperform temporal, multi-stage, and single-stage state-of-the-art methods. Numbers are in mm.} %\phuang{Add \cite{li2021hybrik,lin2021metro}?}}
    \label{tab:sota_3dpw}
    \vspace{-2ex}
\end{table}{}

% \begin{table}[t]
% 	\centering
% 	\resizebox{0.42\textwidth}{!}{
% 		\begin{tabular}{ll|r|r|r}
% 			\toprule
% 			& & \multicolumn{3}{c}{ \threedpw }  \\
% 			\cmidrule(lr){3-5}
% 			& \bf Method & MPJPE $\downarrow$ & PA-MPJPE $\downarrow$ & PVE $\downarrow$\\
% 			\midrule
% 			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{multi stage}}} & Pose2Mesh~\cite{Choi_2020_ECCV_Pose2Mesh} & 88.9 & 58.3 & - \\
% 			& Zanfir~\etal~\cite{zanfir2020weakly} & 90.0 & 57.1 & - \\
% 			& I2L-MeshNet~\cite{Moon_2020_ECCV_I2L-MeshNet} & 93.2 & 57.7 & - \\
% 			% & I2L-MeshNet\textsuperscript{\textdagger}~\cite{Moon_2020_ECCV_I2L-MeshNet} & 100.0 & 60.7  \\
% 			& LearnedGD~\cite{song2020human} & - & 56.4  & - \\
% 			\midrule
% 			\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{single stage}}} & HMR~\cite{kanazawa_hmr} & 130.0 & 76.7 & -  \\
% 			& CMR~\cite{kolotouros2019cmr} & - & 70.2 & - \\
% 			& SPIN~\cite{SPIN:ICCV:2019} & 96.9 & 59.2 & 135.1 \\
% 			& HMR-EFT~\cite{joo2020eft} & - & 54.2 & - \\
% 			\cmidrule(lr){2-5}
% 			& PARE (R50) & \textbf{79.8} & 48.5 & \textbf{96.6} \\
% 			& PARE (HRNet-W32) & 80.8 & \textbf{46.9} & 96.9 \\
% 			\bottomrule
% 		\end{tabular} 
% 	}
% 	\caption{\textbf{Evaluation on the \threedpw dataset.} The numbers are average joint errors in mm. PARE models outperform both multi-stage and single-stage state-of-the-art methods.}
%     \label{tab:sota_3dpw}
%     \vspace{-2ex}
% \end{table}{}

==> tables/table_2_3dpw-occ_sota.tex <==
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{l|r|r|r|r|r}
			\toprule
			& \multicolumn{3}{c|}{ \threedpwocc } & \multicolumn{2}{c}{ \ooh } \\
			\cmidrule(lr){2-6}
			\textbf{Method} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} \\
			\midrule
			Zhang~\etal~\cite{zhangoohcvpr20} & - & 72.2 & - & - & 58.5 \\
			SPIN~\cite{SPIN:ICCV:2019} & 98.4 & 62.5 & 135.1 & 104.3 & 68.3 \\
			HMR-EFT~\cite{joo2020eft} & 95.8 & 62.0 & 120.5 & 75.2 & 53.1 \\
			\midrule
			PARE (R50) & \bf 91.4 & \bf 57.4 & \bf 115.3 & \bf 63.3 & \bf 44.3 \\
			\bottomrule
		\end{tabular} 
	}
	\vspace{-0.05in}
	\caption{\textbf{Evaluation on occlusion datasets \threedpwocc, \ooh}. Here all methods except SPIN are trained with the same datasets, \ie~\coco, \hthreesixm and \ooh. % for a fair comparison.
	}
	\label{tab:sota_occ}
	\vspace{-2ex}
\end{table}{}

% \begin{table}[t]
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 		\begin{tabular}{l|r|r|r|r|r}
% 			\toprule
% 			& \multicolumn{3}{c}{ \threedpwocc } & \multicolumn{2}{c}{ \ooh } \\
% 			\cmidrule(lr){2-6}
% 			\textbf{Method} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} \\
% 			\midrule
% 			Zhang~\etal~\cite{zhangoohcvpr20} & - & 72.2 & - & - & 58.5 \\
% 			SPIN~\cite{SPIN:ICCV:2019} & 98.22 & 60.6 & 135.1 & 104.3 & 68.3 \\
% 			HMR-EFT~\cite{joo2020eft} & 95.2 & 60.2 & 119.5 & 75.2 & 53.1 \\
% 			\midrule
% 			PARE (R50) & \textbf{91.0} & \textbf{55.9} & \textbf{114.1} & \bf 63.3 & \bf 44.3 \\
% 			\bottomrule
% 		\end{tabular} 
% 	}
% 	\caption{\textbf{Evaluation on occlusion datasets \threedpwocc, \ooh}. Here all methods except SPIN are trained with the same datasets, \ie~\coco, \hthreesixm and \ooh. % for a fair comparison.
% 	}
% 	\label{tab:sota_occ}
% \end{table}{}

==> tables/table_3_ablation.tex <==
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{ll|r|r|r|r}
			\toprule %https://www.overleaf.com/project/5f4ac31356c62e0001f3ad6d
			& & \multicolumn{2}{c|}{ \threedpw } & \multicolumn{2}{c}{ \threedpwocc } \\
			\cmidrule{3-6}
			\textbf{Method} & & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} \\
			\midrule
			\rowcolor{pink} & NBF~\cite{omran2018nbf} & 101.8 & 61.1 & 104.6 & 71.1 \\
			& HMR-EFT & 100.4 & 58.7 & 99.2 & 65.7 \\
			\midrule
			\bf $P$ Supervision & \bf $F$ Sampling & \multicolumn{4}{c}{}  \\
			\midrule
			(a) Joints & Pooling & 97.5 & 58.1 & 96.7 & 64.2 \\
			(b) Joints & Attention & 98.2 & 57.7 & 100.4 & 64.8 \\
			\midrule
			% Ours + Parts + Attention & 97.48 & 56.42 & 96.47 & 62.47 \\
			(c) Unsup & Attention & 97.6 & 57.0 & 98.0 & 63.9 \\
			% Ours + Parts/Unsup + Attention & 97.46 & 56.67 & 96.07 & 63.17 \\
			(d) Parts & Attention & 96.9 & 56.3 & 96.3 & \bf 62.2 \\
			(e) Parts/Unsup & Attention & \bf 95.9 & \bf 56.0 & \bf 95.6 & 62.6 \\
			\rowcolor{pink} (f) Parts & Pooling & 99.9 & 58.0 & 101.1 & 65.8 \\
			% \midrule
			% Ours + upsample + nonlocal & & & & \\
			\bottomrule
		\end{tabular} 
	}
	\caption{\textbf{\textcolor{blue}{Exploring} part attention.} %Here we show how part attention evolves. 
	The ``$P$ Supervision" column shows the type of supervision for the 2D part branch $P$. ``$F$ Sampling" shows the type of feature sampling method for $F$. All methods are trained on \cocoeft with a ResNet-50 backbone.}
	\vspace{-3ex}
	\label{tab:ablation_attention}

\end{table}{}

% \begin{table}[t]
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 	\begin{tabular}{ll|r|r|r|r|r|r}
% 			\toprule %https://www.overleaf.com/project/5f4ac31356c62e0001f3ad6d
% 			& & \multicolumn{3}{c|}{ \threedpw } & \multicolumn{3}{c}{ \threedpwocc } \\
% 			\cmidrule{3-8}
% 			\textbf{Method} & & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} \\
% 			\midrule
% 			& HMR-EFT & 98.5 & 56.3 & 115.3 & 99.0 & 63.9 & 121.4 \\
% 			\midrule
% 			\bf $P$ Supervision & \bf $F$ Sampling & \multicolumn{6}{c}{}  \\
% 			\midrule
% 			(a) Joints & Pooling & 94.1 & 55.1 & 111.2 & 96.4 & 62.4 & 118.8 \\
% 			(b) Joints & Attention & 95.7 & 54.7 & 114.1 & 100.5 & 63.0 & 124.9 \\
% 			\midrule
% 			(c) Unsup & Attention & 94.6 & 53.9 & 112.5 & 97.8 & 62.3 & 120.7 \\
% 			(d) Parts & Attention & 93.7 & 53.2 & 110.2 & 96.2 & \textbf{60.4} & 119.0 \\
% 			(e) Parts/Unsup & Attention & \textbf{92.5} & \textbf{53.0} & \textbf{109.5} & \textbf{95.6} & 61.0 & \textbf{118.6} \\
% 			\bottomrule
% 		\end{tabular} 
% 	}
% 	\caption{\textbf{Evolution of part attention.} Here we show how part attention evolves. The ``$P$ Supervision" column shows the type of supervision for 2D part branch $P$. ``$F$ Sampling" shows the type of feature sampling method for $F$. All methods are trained on \cocoeft with a ResNet-50 backbone.}
% 	\label{tab:ablation_attention}
% 	\vspace{-2ex}
% \end{table}{}

==> tables/table_4_ablation_occ-aug.tex <==
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{
	    \begin{tabular}{l|r|r|r|r}
	    \toprule
        & \multicolumn{2}{c|}{ \threedpw } & \multicolumn{2}{c}{ \threedpwocc } \\
        \cmidrule{2-5}
        \textbf{Method} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} \\
        \midrule
        % HMR-EFT & 99.0 & 58.6 & 100.3 & 67.0 \\
        HMR-EFT + SynthOcc & 100.4 & 58.7 & 99.2 & 65.7 \\
        % HMR-EFT + synth + crop & 98.6 & 58.3 & 97.8 & 65.5 \\
        \midrule
        PARE & 98.2 & 56.8 & 96.4 & 62.4 \\
        PARE + SynthOcc & \bf 96.9 & \bf 56.3 & \bf 96.3 & \bf 62.2 \\
        PARE + SynthOcc + RandCrop & 98.9 & 56.8 & 99.1 & 63.1 \\
        % PARE + COCO-SynthOcc & 99.5 & 57.2 & 97.9 & 63.7 \\
        \bottomrule
        \end{tabular} 
	}	
	\vspace{-0.05in}
	\caption{\textbf{Ablation of different occlusion augmentation strategies.} We demonstrate the effect of synthetic occlusion (SynthOcc) and random crop (RandCrop) augmentation on the final performance. All methods are trained on \cocoeft with ResNet-50 as the backbone.}
	\label{tab:ablation_occ}
	\vspace{-3ex}
\end{table}{}

% \begin{table}[t]
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 	    \begin{tabular}{l|r|r|r|r|r|r}
% 	    \toprule
%         & \multicolumn{3}{c}{ \threedpw } & \multicolumn{3}{c}{ \threedpwocc } \\
%         \cmidrule{2-7}
%         \textbf{Method} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} \\
%         \midrule
%         HMR-EFT & 98.5 & 56.3 & 115.3 & 99.0 & 63.9 & 121.4 \\
%         \midrule
%         PARE & 95.3 & 53.8 & 112.0 & 96.8 & 60.7 & 120.2 \\
%         PARE + SynthOcc & \textbf{93.7} & \textbf{53.2} & \textbf{110.2} & \textbf{96.2} & \textbf{60.4} & \textbf{119.0} \\
%         PARE + SynthOcc + RandCrop & 98.6 & 54.1 & 116.4 & 100.5 & 61.6 & 127.4 \\
%         PARE + COCO-SynthOcc & 96.5 & 54.3 & 114.4 & 97.8 & 62.1 & 121.3 \\
%         \bottomrule
%         \end{tabular} 
% 	}
% 	\vspace{-2ex}
% 	\caption{\textbf{Ablation of different occlusion augmentation strategies.} We demonstrate the effect of synthetic occlusion (SynthOcc) and random crop (RandCrop) augmentation on the final performance. All methods are trained on \cocoeft with ResNet-50 as the backbone.}
% 	\label{tab:ablation_occ}
% 	\vspace{-2ex}
% \end{table}{}

==> tables/table_5_ablation_backbone.tex <==
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{
	    \begin{tabular}{l|l|r|r|r|r}
	    \toprule
        \multicolumn{2}{c|}{ } & \multicolumn{2}{c|}{ \threedpw } & \multicolumn{2}{c}{ \threedpwocc } \\
        \cmidrule{3-6}
        \multicolumn{2}{l|}{\textbf{Method}} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} \\
        \midrule
        HMR-EFT & ResNet-50 & 100.4 & 58.7 & 99.2 & 65.8 \\
        PARE & ResNet-50 & \bf 95.9 & \bf 56.0 & \bf 95.6 & \bf 62.6 \\
        \midrule
        HMR-EFT & HRNet-W32  & 94.6 & 54.3 & 91.2 & 58.2 \\
        PARE & HRNet-W32 & \bf 92.0 & \bf 53.4 & \bf 88.6 & \bf 57.7 \\
        \bottomrule
        \end{tabular} 
	}
	\vspace{-0.05in}
	\caption{\textbf{Ablation of backbone architectures}. All methods are trained on \cocoeft.}
	\label{tab:ablation_backbone}
	\vspace{-3ex}
\end{table}{}

% \begin{table}[t]
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 	    \begin{tabular}{l|l|r|r|r|r|r|r}
% 	    \toprule
%         \multicolumn{2}{c|}{ } & \multicolumn{3}{c|}{ \threedpw } & \multicolumn{3}{c}{ \threedpwocc } \\
%         \cmidrule{3-8}
%         \multicolumn{2}{l|}{\textbf{Method}} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} & {\footnotesize MPJPE $\downarrow$} & {\footnotesize PA-MPJPE $\downarrow$} & {\footnotesize PVE $\downarrow$} \\
%         \midrule
%         HMR-EFT & ResNet-50 & 98.5 & 56.3 & 115.3 & 99.0 & 63.9 & 121.4 \\
%         PARE & ResNet-50 & \textbf{93.7} & \textbf{53.2} & \textbf{110.2} & \textbf{96.2} & \textbf{60.4} & \textbf{119.0} \\
%         \midrule
%         HMR-EFT & HRNet-W32  & 91.4 & 51.4 & 107.3 & 91.3 & 56.9 & 113.5 \\
%         PARE & HRNet-W32 & 89.4 & 50.6 & 106.5 & 89.2 & 56.2 & 113.3 \\
%         \bottomrule
%         \end{tabular} 
% 	}
% 	\caption{\textbf{Ablation of backbone architectures}. All methods are trained on \cocoeft.}
% 	\label{tab:ablation_backbone}
% 	\vspace{-2ex}
% \end{table}{}
